MEND: RL For Flow Models via Proximal Velocity Matching

Reward post-training of flow models either reweights the model's own samples under a KL penalty or a frozen reference, often for thousands of updates, or backpropagates the reward and moves every sample without checking that the move is worth its size. We introduce MEND, a reinforcement learning method built on proximal velocity matching. MEND caps rewards within each prompt group, so samples that already score well receive no move. Below the cap, it proposes moves along the reward gradient and accepts one only when its capped reward gain exceeds a quadratic displacement price. The model then regresses onto the resulting velocity targets, with no KL term, frozen reference model, or advantage weights. In 100 updates, MEND outperforms Flow-GRPO (about 4k updates) on five of six evaluators at the same distance to base-model images. Under an equal-budget protocol, it surpasses ReFL and DiffusionNFT at every evaluated update across four training rewards, reaching PickScore 24.03 versus 23.92 and 23.43, respectively. A 300-update three-reward run also surpasses the five-reward DiffusionNFT model on all three rewards it trains on. MEND is general and easy to adopt: it applies to any flow backbone with a differentiable reward.

==> figures/snippets/v2_fig_frontier_a.tex <==
\begin{minipage}[t]{0.48\linewidth}
\vspace{0pt}
\centering
\mendfig{v2/fig_frontier_a.pdf}{\linewidth}{1.9in}{PickScore against distance to the pre-trained images}
\caption{\textbf{Higher reward, closer to the pre-trained model.} PickScore against DreamSim distance to the pre-trained images along training (DrawBench $200\times5$; numbers mark updates). At every update \mend{} is above DiffusionNFT under the same protocol and closer to the pre-trained images.}
\label{fig:frontier-main}
\end{minipage}


==> figures/snippets/v2_fig_frontier_b.tex <==
\begin{minipage}[t]{0.48\linewidth}
\vspace{0pt}
\centering
\mendfig{v2/fig_frontier_b.pdf}{\linewidth}{1.9in}{PickScore against diversity}
\caption{\textbf{Higher reward at equal diversity.} PickScore against DreamSim diversity along training (DrawBench $200\times5$; numbers mark updates). At equal diversity \mend{} is at least 0.35 above DiffusionNFT under the same protocol.}
\label{fig:frontier-div}
\end{minipage}


==> figures/snippets/v2_fig_overopt.tex <==
\begin{figure}[!htbp]
\centering
\mendfig{v2/fig_overopt.pdf}{\linewidth}{1.62in}{Training past the budget: five metrics against updates}
\caption{\textbf{Training past the budget.} A second PickScore run trained for 200 updates; each panel shows the change from the base relative to the change at update 100 (dotted line). The trained reward keeps rising while held-out gains flatten and HPSv3 peaks at update 60.}
\label{fig:campaign-overopt}
\end{figure}


==> figures/v2/prompts_v2.tex <==

\noindent\textbf{Figure~\ref{fig:hero}, top part, columns left to right.} (1) seed 0: ``A lighthouse on a cliff to the left and a sailboat to the right on a calm sea, a full moon between them, blue hour.''; (2) seed 45: ``Four dogs on the street.''; (3) seed 43: ``A small blue book sitting on a large red book.''; (4) seed 1: ``A miniature train set winding through a handmade model town with tiny people, trees and street lamps, tilt-shift photograph.''; (5) seed 0: ``A steaming bowl of ramen with a soft-boiled egg, sliced pork, scallions and nori, dark wooden table, moody food photography.''.

\noindent\textbf{Figure~\ref{fig:cmp}, rows top to bottom.} (1) seed 0: ``A cat wearing a tiny knitted scarf sitting inside a teacup, next to a stack of three books, cozy window light.''; (2) seed 1: ``A cute ceramic dragon figurine with glossy teal glaze, isometric 3D render, soft pastel background, clay material.''; (3) seed 1: ``Close-up of a peacock feather showing iridescent blue and green barbules, studio macro, black background.''; (4) seed 0: ``A giant tortoise carrying a small village with tiny houses and trees on its shell, walking through a shallow sea, fantasy illustration.''; (5) seed 42: ``multidimensional quantum foam realm brane fantasy style''.

\noindent\textbf{Figure~\ref{fig:fidelity}, columns left to right.} (1) seed 42: ``An umbrella on top of a spoon.''; (2) seed 43: ``A tennis racket underneath a traffic light.''; (3) seed 46: ``Three dogs on the street.''; (4) seed 42: ``A yellow book and a red vase.''; (5) seed 46: ``A green apple and a black backpack.''; (6) seed 45: ``A bird scaring a scarecrow.''.

\noindent\textbf{Figure~\ref{fig:progress}, rows top to bottom.} (1) seed 45: ``A spider with a moustache bidding an equally gentlemanly grasshopper a good day during his walk to work.''; (2) seed 43: ``A medieval painting of the wifi not working.''.

\noindent\textbf{Figure~\ref{fig:qual}, columns left to right.} (1) seed 1: ``Desert canyon with glowing red sandstone walls at dusk, a thunderstorm on the horizon with a single lightning bolt, wide-angle photograph.''; (2) seed 0: ``An ancient tree with a glowing door carved into its trunk, fireflies and luminous mushrooms around its roots, enchanted night forest.''; (3) seed 43: ``A badge, flag , icon, space, space program,''; (4) seed 0: ``Ornate sapphire tiara in a dim museum vitrine, blue stones and diamonds sparkling under spotlight with glass reflections.''; (5) seed 42: ``a treehouse on a palm tree''; (6) seed 1: ``A chef's hands dusting flour over fresh handmade pasta on a wooden board, flour particles in the air, side light.''.

\noindent\textbf{Figure~\ref{fig:cmp2}, rows top to bottom.} (1) seed 0: ``Looking up at a spiral staircase inside an old library with carved wooden railings and shelves of leather-bound books on every floor.''; (2) seed 0: ``Surreal commuter, a man wearing a crossbody bag, calmly walking through a doorway cut into a frozen ocean wave, with impossible physics and cinematic light.''; (3) seed 0: ``A red panda curled up asleep on a mossy branch, soft morning fog in a bamboo forest.''; (4) seed 1: ``A lone wooden cabin on the shore of a frozen lake under a sky full of green and violet northern lights, reflections on the ice, long exposure.''.

\noindent\textbf{Figure~\ref{fig:progress-main}, rows top to bottom.} (1) seed 46: ``A triangular purple flower pot. A purple flower pot in the shape of a triangle.''; (2) seed 43: the same prompt.

\noindent\textbf{Figure~\ref{fig:cmp-more}, rows top to bottom.} (1) seed 42: ``cat astronaut, in space, psychedelic, cosmic''; (2) seed 0: ``Cinque Terre-style Italian coastal village with colorful cliff houses, turquoise sea, boats, laundry lines and warm afternoon light.''; (3) seed 0: ``A towering waterfall plunging into a jungle gorge, a rainbow in the spray, tiny rope bridge crossing in the foreground, lush ferns.''; (4) seed 0: ``A floating island with a waterfall pouring off its edge into the clouds below, a small castle on top, airships in the sky, epic matte painting.''.

\noindent\textbf{Figure~\ref{fig:qual-more}, columns left to right.} (1) seed 0: ``High-speed macro of a water-droplet crown frozen mid-splash on a colorful surface, elegant and detailed.''; (2) seed 1: ``A fox reading a book under an oak tree in autumn, children's book watercolor illustration, soft washes and visible paper texture.''; (3) seed 42: ``a chubby goblin juggling rubber balls''; (4) seed 1: ``Miniature explorer camp on a mossy log imagined as a vast landscape, with dramatic macro lighting and a tiny explorer in the scene.''; (5) seed 0: ``A ballerina mid-leap on an empty theater stage lit by a single spotlight, motion-blurred tulle skirt, dust particles floating in the light beam.''; (6) seed 43: ``close up photo of a rabbit, forest, haze, halation, bloom, dramatic atmosphere, centred, rule of thirds, 200mm 1.4f macro shot''.


==> results.tex <==
\makeatletter
\newcommand{\setres}[2]{\if\relax\detokenize{#2}\relax\else\expandafter\def\csname mres@#1\endcsname{#2}\fi}
\newcommand{\setest}[2]{\expandafter\def\csname mest@#1\endcsname{#2}}
\newcommand{\res}[1]{\ifcsname mres@#1\endcsname\csname mres@#1\endcsname\else\ifcsname mest@#1\endcsname\ph{\csname mest@#1\endcsname}\else\tbd\fi\fi}
\newcommand{\resrow}[1]{\res{#1.pick} & \res{#1.hps2} & \res{#1.hps3} & \res{#1.ir} & \res{#1.clip} & \res{#1.aes} & \res{#1.div} & \res{#1.dist}}
\newcommand{\resrowhf}[1]{\res{#1.pick} & \res{#1.hps2} & \res{#1.hps3} & \res{#1.ir} & \res{#1.clip} & \res{#1.aes} & \res{#1.div} & \res{#1.hf}}
\newcommand{\genevalrow}[1]{\res{#1.single} & \res{#1.two} & \res{#1.count} & \res{#1.colors} & \res{#1.pos} & \res{#1.attr} & \res{#1.overall}}
\providecommand{\resph}[2]{\ifcsname mres@#1\endcsname\csname mres@#1\endcsname\else\ph{#2}\fi}
\makeatother
\setres{gbase1.single}{0.80}\setres{gbase1.two}{0.30}\setres{gbase1.count}{0.18}\setres{gbase1.colors}{0.49}\setres{gbase1.pos}{0.07}\setres{gbase1.attr}{0.10}\setres{gbase1.overall}{0.32}
\setres{gbase45.single}{0.99}\setres{gbase45.two}{0.84}\setres{gbase45.count}{0.59}\setres{gbase45.colors}{0.82}\setres{gbase45.pos}{0.24}\setres{gbase45.attr}{0.57}\setres{gbase45.overall}{0.68}
\setres{gfgge.single}{1.00}\setres{gfgge.two}{0.99}\setres{gfgge.count}{0.94}\setres{gfgge.colors}{0.91}\setres{gfgge.pos}{0.94}\setres{gfgge.attr}{0.84}\setres{gfgge.overall}{0.94}
\setres{gnft.single}{1.00}\setres{gnft.two}{0.99}\setres{gnft.count}{0.88}\setres{gnft.colors}{0.95}\setres{gnft.pos}{0.92}\setres{gnft.attr}{0.86}\setres{gnft.overall}{0.93}
\setres{obase1.ocr}{0.13}\setres{obase45.ocr}{0.57}\setres{ofgtext.ocr}{0.91}\setres{onft.ocr}{0.92}
\setres{rwdefimagerewardc80.ir}{1.27}
\setres{gbase1.pub}{0.24}\setres{gbase45.pub}{0.62}\setres{gnft.pub}{0.93}\setres{gfgge.pub}{0.95}
\setres{rwhpsv2pre.pick}{23.01}\setres{rwhpsv2pre.hps2}{0.358}\setres{rwhpsv2pre.hps3}{7.23}\setres{rwhpsv2pre.ir}{1.20}\setres{rwhpsv2pre.clip}{0.267}\setres{rwhpsv2pre.aes}{5.88}\setres{rwhpsv2pre.div}{0.184}\setres{rwhpsv2pre.dist}{0.519}\setres{rwhpsv2pre.hf}{0.82}
\setres{zbase.dist}{0}
\InputIfFileExists{results_data.tex}{}{}
\newcommand{\mPick}{\res{fin.pick}}
\newcommand{\mDiv}{\res{fin.div}}
\newcommand{\mDist}{\res{fin.dist}}
\newcommand{\mClip}{\res{fin.clip}}
\newcommand{\mHPSt}{\res{fin.hps2}}
\newcommand{\mHPSthree}{\res{fin.hps3}}
\newcommand{\mIR}{\res{fin.ir}}
\newcommand{\mAes}{\res{fin.aes}}
\newcommand{\mCFG}{4.5}
\newcommand{\mgPick}{\res{cfg45.pick}}
\newcommand{\mgDiv}{\res{cfg45.div}}
\newcommand{\mgDist}{\res{cfg45.dist}}
\newcommand{\mgClip}{\res{cfg45.clip}}
\setest{cfg3.pick}{23.82}\setest{cfg3.hps2}{0.317}\setest{cfg3.hps3}{6.4}\setest{cfg3.ir}{1.26}\setest{cfg3.clip}{0.287}\setest{cfg3.aes}{5.96}\setest{cfg3.div}{0.156}\setest{cfg3.dist}{0.52}\setest{cfg3.hf}{0.85}
\setest{cfg45.pick}{23.52}\setest{cfg45.hps2}{0.315}\setest{cfg45.hps3}{6.3}\setest{cfg45.ir}{1.22}\setest{cfg45.clip}{0.287}\setest{cfg45.aes}{5.86}\setest{cfg45.div}{0.160}\setest{cfg45.dist}{0.52}\setest{cfg45.hf}{0.9}
\setest{ccfg45.pick}{23.61}\setest{ccfg45.hps2}{0.319}\setest{ccfg45.hps3}{6.4}\setest{ccfg45.ir}{1.30}\setest{ccfg45.clip}{0.288}\setest{ccfg45.aes}{5.93}\setest{ccfg45.div}{0.142}\setest{ccfg45.dist}{0.52}\setest{ccfg45.hf}{0.88}
\setest{ccfg2.pick}{24.15}\setest{ccfg2.hps2}{0.319}\setest{ccfg2.hps3}{6.2}\setest{ccfg2.ir}{1.35}\setest{ccfg2.clip}{0.288}\setest{ccfg2.aes}{6.10}\setest{ccfg2.div}{0.150}\setest{ccfg2.dist}{0.51}\setest{ccfg2.hf}{0.78}
\setest{rwhpsv2pre.hps2}{0.358}\setest{rwhpsv3pre.hps3}{6.1}
\setest{pf.pick}{23.5}\setest{pf.hps2}{0.300}\setest{pf.hps3}{4.6}\setest{pf.ir}{1.02}\setest{pf.clip}{0.277}\setest{pf.aes}{5.80}\setest{pf.div}{0.23}\setest{pf.dist}{0.33}\setest{pf.hf}{0.95}
\newcommand{\iPick}{23.90}
\newcommand{\iHPSt}{0.298}
\newcommand{\iHPSthree}{3.75}
\newcommand{\iIR}{1.07}
\newcommand{\iClip}{0.271}
\newcommand{\iAes}{6.18}
\newcommand{\iDiv}{0.212}
\newcommand{\iDist}{0.491}
\newcommand{\iHF}{0.49}

\setres{base.pick}{22.35}
\setres{base.hps2}{0.280}
\setres{base.hps3}{2.72}
\setres{base.ir}{0.83}
\setres{base.clip}{0.283}
\setres{base.aes}{5.39}
\setres{base.dist}{0}
\setres{flow.pick}{23.52}
\setres{flow.hps2}{0.316}
\setres{flow.hps3}{7.04}
\setres{flow.ir}{1.27}
\setres{flow.clip}{0.280}
\setres{flow.aes}{5.90}
\setres{flow.dist}{0.313}
\setres{nft.pick}{23.82}
\setres{nft.hps2}{0.331}
\setres{nft.hps3}{7.50}
\setres{nft.ir}{1.49}
\setres{nft.clip}{0.292}
\setres{nft.aes}{6.02}
\setres{nft.dist}{0.538}
\setres{refl.pick}{23.92}
\setres{refl.ir}{1.28}
\setres{refl.hps2}{0.358}
\setres{refl.clip}{0.308}
\setres{nftequal.pick}{23.43}
\setres{nftequal.ir}{1.46}
\setres{nftequal.hps2}{0.336}
\setres{nftequal.clip}{0.298}
\setres{sd3base.pick}{20.36}
\setres{sd3base.hps2}{0.215}
\setres{sd3mend.pick}{23.70}
\setres{sd3mend.hps2}{0.298}
\setres{sd3dpo.pick}{20.96}
\setres{sd3dpo.hps2}{0.256}
\setres{flow.updates}{4k}
\setres{nft.updates}{1.7k}
\setres{base.updates}{0}
\setres{train.gpuh}{10.0}
\setres{update.ratio}{40}
\setres{early.update}{25}
\setres{qual.res}{1024}
\setres{nft.pickgap}{0.12}
\setres{abref.moved}{34\%}
\setres{abnocap.moved}{45\%}
\setres{abnoprice.moved}{78\%}
\setres{abkone.moved}{37\%}
\setres{abnvtwo.moved}{81\%}


==> results_data.tex <==
\setres{fin.pick}{24.03}
\setres{fin.hps2}{0.301}
\setres{fin.hps3}{3.71}
\setres{fin.ir}{1.13}
\setres{fin.clip}{0.273}
\setres{fin.aes}{6.24}
\setres{fin.div}{0.202}
\setres{fin.dist}{0.495}
\setres{fin.hf}{0.54}
\setres{u200.pick}{24.22}
\setres{u200.hps2}{0.304}
\setres{u200.hps3}{3.70}
\setres{u200.ir}{1.19}
\setres{u200.clip}{0.274}
\setres{u200.aes}{6.24}
\setres{u200.div}{0.181}
\setres{u200.dist}{0.497}
\setres{u200.hf}{0.57}
\setres{cfin.pick}{24.12}
\setres{cfin.hps2}{0.304}
\setres{cfin.hps3}{3.82}
\setres{cfin.ir}{1.21}
\setres{cfin.clip}{0.274}
\setres{cfin.aes}{6.31}
\setres{cfin.div}{0.184}
\setres{cfin.dist}{0.490}
\setres{cfin.hf}{0.52}
\setres{finval.pick}{24.07}
\setres{finval.div}{0.140}
\setres{finclean.pick}{24.12}
\setres{finclean.div}{0.184}
\setres{fin.moved}{0.37}
\setres{cfg2.pick}{24.06}
\setres{cfg2.hps2}{0.316}
\setres{cfg2.hps3}{6.12}
\setres{cfg2.ir}{1.27}
\setres{cfg2.clip}{0.287}
\setres{cfg2.aes}{6.03}
\setres{cfg2.div}{0.165}
\setres{cfg2.dist}{0.514}
\setres{cfg2.hf}{0.79}
\setres{cfg3.pick}{23.92}
\setres{cfg3.hps2}{0.319}
\setres{cfg3.hps3}{6.84}
\setres{cfg3.ir}{1.30}
\setres{cfg3.clip}{0.290}
\setres{cfg3.aes}{5.95}
\setres{cfg3.div}{0.149}
\setres{cfg3.dist}{0.527}
\setres{cfg3.hf}{1.03}
\setres{cfg45.pick}{23.70}
\setres{cfg45.hps2}{0.319}
\setres{cfg45.hps3}{7.15}
\setres{cfg45.ir}{1.32}
\setres{cfg45.clip}{0.291}
\setres{cfg45.aes}{5.88}
\setres{cfg45.div}{0.144}
\setres{cfg45.dist}{0.313}
\setres{cfg45.hf}{1.36}
\setres{cfg45c025.pick}{23.36}
\setres{cfg45c025.hps2}{0.312}
\setres{cfg45c025.hps3}{6.69}
\setres{cfg45c025.ir}{1.18}
\setres{cfg45c025.clip}{0.284}
\setres{cfg45c025.aes}{5.85}
\setres{cfg45c025.div}{0.177}
\setres{cfg45c025.dist}{0.294}
\setres{cfg45c025.hf}{1.13}
\setres{cfg45c050.pick}{23.55}
\setres{cfg45c050.hps2}{0.318}
\setres{cfg45c050.hps3}{7.17}
\setres{cfg45c050.ir}{1.29}
\setres{cfg45c050.clip}{0.288}
\setres{cfg45c050.aes}{5.89}
\setres{cfg45c050.div}{0.157}
\setres{cfg45c050.dist}{0.308}
\setres{cfg45c050.hf}{1.27}
\setres{cfg45c075.pick}{23.64}
\setres{cfg45c075.hps2}{0.319}
\setres{cfg45c075.hps3}{7.08}
\setres{cfg45c075.ir}{1.32}
\setres{cfg45c075.clip}{0.290}
\setres{cfg45c075.aes}{5.88}
\setres{cfg45c075.div}{0.147}
\setres{cfg45c075.dist}{0.311}
\setres{cfg45c075.hf}{1.29}
\setres{ccfg45.pick}{23.75}
\setres{ccfg45.hps2}{0.322}
\setres{ccfg45.hps3}{7.30}
\setres{ccfg45.ir}{1.34}
\setres{ccfg45.clip}{0.291}
\setres{ccfg45.aes}{5.95}
\setres{ccfg45.div}{0.143}
\setres{ccfg45.dist}{0.311}
\setres{ccfg45.hf}{1.34}
\setres{sw1.pick}{24.06}
\setres{sw1.hps2}{0.315}
\setres{sw1.ir}{1.29}
\setres{sw1.clip}{0.278}
\setres{sw1.aes}{6.60}
\setres{sw1.div}{0.140}
\setres{swk1.pick}{24.00}
\setres{swk1.hps2}{0.316}
\setres{swk1.ir}{1.30}
\setres{swk1.clip}{0.284}
\setres{swk1.aes}{6.54}
\setres{swk1.div}{0.155}
\setres{sw15.pick}{24.04}
\setres{sw15.hps2}{0.322}
\setres{sw15.ir}{1.36}
\setres{sw15.clip}{0.290}
\setres{sw15.aes}{6.52}
\setres{sw15.div}{0.115}
\setres{swk15.pick}{23.94}
\setres{swk15.hps2}{0.323}
\setres{swk15.ir}{1.37}
\setres{swk15.clip}{0.289}
\setres{swk15.aes}{6.43}
\setres{swk15.div}{0.136}
\setres{sw2.pick}{23.93}
\setres{sw2.hps2}{0.325}
\setres{sw2.ir}{1.42}
\setres{sw2.clip}{0.293}
\setres{sw2.aes}{6.43}
\setres{sw2.div}{0.109}
\setres{swk2.pick}{23.85}
\setres{swk2.hps2}{0.325}
\setres{swk2.ir}{1.41}
\setres{swk2.clip}{0.291}
\setres{swk2.aes}{6.34}
\setres{swk2.div}{0.126}
\setres{sw25.pick}{23.82}
\setres{sw25.hps2}{0.327}
\setres{sw25.ir}{1.40}
\setres{sw25.clip}{0.293}
\setres{sw25.aes}{6.39}
\setres{sw25.div}{0.104}
\setres{swk25.pick}{23.75}
\setres{swk25.hps2}{0.325}
\setres{swk25.ir}{1.42}
\setres{swk25.clip}{0.291}
\setres{swk25.aes}{6.31}
\setres{swk25.div}{0.115}
\setres{sw3.pick}{23.68}
\setres{sw3.hps2}{0.326}
\setres{sw3.ir}{1.41}
\setres{sw3.clip}{0.293}
\setres{sw3.aes}{6.36}
\setres{sw3.div}{0.102}
\setres{swk3.pick}{23.65}
\setres{swk3.hps2}{0.325}
\setres{swk3.ir}{1.41}
\setres{swk3.clip}{0.294}
\setres{swk3.aes}{6.29}
\setres{swk3.div}{0.116}
\setres{sw35.pick}{23.58}
\setres{sw35.hps2}{0.326}
\setres{sw35.ir}{1.39}
\setres{sw35.clip}{0.292}
\setres{sw35.aes}{6.33}
\setres{sw35.div}{0.098}
\setres{swk35.pick}{23.54}
\setres{swk35.hps2}{0.325}
\setres{swk35.ir}{1.40}
\setres{swk35.clip}{0.293}
\setres{swk35.aes}{6.25}
\setres{swk35.div}{0.117}
\setres{sw4.pick}{23.50}
\setres{sw4.hps2}{0.326}
\setres{sw4.ir}{1.39}
\setres{sw4.clip}{0.292}
\setres{sw4.aes}{6.29}
\setres{sw4.div}{0.104}
\setres{swk4.pick}{23.45}
\setres{swk4.hps2}{0.325}
\setres{swk4.ir}{1.41}
\setres{swk4.clip}{0.294}
\setres{swk4.aes}{6.24}
\setres{swk4.div}{0.117}
\setres{sw45.pick}{23.39}
\setres{sw45.hps2}{0.325}
\setres{sw45.ir}{1.36}
\setres{sw45.clip}{0.293}
\setres{sw45.aes}{6.26}
\setres{sw45.div}{0.104}
\setres{swk45.pick}{23.38}
\setres{swk45.hps2}{0.325}
\setres{swk45.ir}{1.41}
\setres{swk45.clip}{0.296}
\setres{swk45.aes}{6.21}
\setres{swk45.div}{0.116}
\setres{rwclipscore.pick}{22.27}
\setres{rwclipscore.hps2}{0.268}
\setres{rwclipscore.hps3}{1.15}
\setres{rwclipscore.ir}{0.98}
\setres{rwclipscore.clip}{0.314}
\setres{rwclipscore.aes}{5.22}
\setres{rwclipscore.div}{0.287}
\setres{rwclipscore.dist}{0.450}
\setres{rwclipscore.hf}{0.42}
\setres{rwhpsv2.pick}{23.06}
\setres{rwhpsv2.hps2}{0.360}
\setres{rwhpsv2.hps3}{7.12}
\setres{rwhpsv2.ir}{1.21}
\setres{rwhpsv2.clip}{0.268}
\setres{rwhpsv2.aes}{5.89}
\setres{rwhpsv2.div}{0.181}
\setres{rwhpsv2.dist}{0.519}
\setres{rwhpsv2.hf}{0.82}
\setres{rwimagereward.pick}{22.33}
\setres{rwimagereward.hps2}{0.303}
\setres{rwimagereward.hps3}{4.78}
\setres{rwimagereward.ir}{1.51}
\setres{rwimagereward.clip}{0.266}
\setres{rwimagereward.aes}{5.99}
\setres{rwimagereward.div}{0.181}
\setres{rwimagereward.dist}{0.535}
\setres{rwimagereward.hf}{0.47}
\setres{rwhpsv245.pick}{22.94}
\setres{rwhpsv245.hps2}{0.343}
\setres{rwhpsv245.hps3}{7.37}
\setres{rwhpsv245.ir}{1.29}
\setres{rwhpsv245.clip}{0.285}
\setres{rwhpsv245.aes}{5.61}
\setres{rwhpsv245.div}{0.148}
\setres{rwhpsv245.dist}{0.328}
\setres{rwhpsv245.hf}{1.29}
\setres{rwclipscore45.pick}{22.58}
\setres{rwclipscore45.hps2}{0.298}
\setres{rwclipscore45.hps3}{5.44}
\setres{rwclipscore45.ir}{1.27}
\setres{rwclipscore45.clip}{0.315}
\setres{rwclipscore45.aes}{5.40}
\setres{rwclipscore45.div}{0.186}
\setres{rwclipscore45.dist}{0.303}
\setres{rwclipscore45.hf}{1.20}
\setres{rwimagereward45.pick}{22.41}
\setres{rwimagereward45.hps2}{0.311}
\setres{rwimagereward45.hps3}{5.53}
\setres{rwimagereward45.ir}{1.51}
\setres{rwimagereward45.clip}{0.284}
\setres{rwimagereward45.aes}{5.61}
\setres{rwimagereward45.div}{0.142}
\setres{rwimagereward45.dist}{0.354}
\setres{rwimagereward45.hf}{1.01}
\setres{rwirpre.pick}{22.22}
\setres{rwirpre.hps2}{0.291}
\setres{rwirpre.hps3}{5.13}
\setres{rwirpre.ir}{1.17}
\setres{rwirpre.clip}{0.259}
\setres{rwirpre.aes}{5.99}
\setres{rwirpre.div}{0.256}
\setres{rwirpre.dist}{0.495}
\setres{rwirpre.hf}{0.61}
\setres{rwclippre.pick}{22.22}
\setres{rwclippre.hps2}{0.265}
\setres{rwclippre.hps3}{1.11}
\setres{rwclippre.ir}{0.87}
\setres{rwclippre.clip}{0.306}
\setres{rwclippre.aes}{5.25}
\setres{rwclippre.div}{0.323}
\setres{rwclippre.dist}{0.425}
\setres{rwclippre.hf}{0.34}
\setres{rwhpsv2pre.pick}{23.01}
\setres{rwhpsv2pre.hps2}{0.358}
\setres{rwhpsv2pre.hps3}{7.23}
\setres{rwhpsv2pre.ir}{1.20}
\setres{rwhpsv2pre.clip}{0.267}
\setres{rwhpsv2pre.aes}{5.88}
\setres{rwhpsv2pre.div}{0.184}
\setres{rwhpsv2pre.dist}{0.519}
\setres{rwhpsv2pre.hf}{0.82}
\setres{opsdpickscore.pick}{24.97}
\setres{opsdpickscore.hps2}{0.311}
\setres{opsdpickscore.hps3}{3.96}
\setres{opsdpickscore.ir}{1.19}
\setres{opsdpickscore.clip}{0.261}
\setres{opsdpickscore.aes}{6.33}
\setres{opsdpickscore.div}{0.142}
\setres{opsdpickscore.dist}{0.524}
\setres{opsdpickscore.hf}{1.34}
\setres{opsdhpsv2.pick}{23.15}
\setres{opsdhpsv2.hps2}{0.391}
\setres{opsdhpsv2.hps3}{8.26}
\setres{opsdhpsv2.ir}{1.33}
\setres{opsdhpsv2.clip}{0.268}
\setres{opsdhpsv2.aes}{6.10}
\setres{opsdhpsv2.div}{0.132}
\setres{opsdhpsv2.dist}{0.538}
\setres{opsdhpsv2.hf}{1.69}
\setres{opsdclipscore.pick}{22.39}
\setres{opsdclipscore.hps2}{0.275}
\setres{opsdclipscore.hps3}{$-$0.43}
\setres{opsdclipscore.ir}{1.06}
\setres{opsdclipscore.clip}{0.341}
\setres{opsdclipscore.aes}{5.32}
\setres{opsdclipscore.div}{0.228}
\setres{opsdclipscore.dist}{0.495}
\setres{opsdclipscore.hf}{0.54}
\setres{opsdhpsv3.pick}{22.48}
\setres{opsdhpsv3.hps2}{0.327}
\setres{opsdhpsv3.hps3}{13.42}
\setres{opsdhpsv3.ir}{1.14}
\setres{opsdhpsv3.clip}{0.269}
\setres{opsdhpsv3.aes}{6.08}
\setres{opsdhpsv3.div}{0.194}
\setres{opsdhpsv3.dist}{0.537}
\setres{opsdhpsv3.hf}{2.95}
\setres{rwdefclipscore.clip}{0.306}
\setres{rwdefhpsv2.hps2}{0.358}
\setres{rwdefimagereward.ir}{1.44}
\setres{o3.pick}{23.89}
\setres{o3.hps2}{0.344}
\setres{o3.hps3}{5.87}
\setres{o3.ir}{1.28}
\setres{o3.clip}{0.300}
\setres{o3.aes}{5.92}
\setres{o3.div}{0.188}
\setres{o3.dist}{0.488}
\setres{o3.hf}{0.82}
\setres{pf.pick}{23.56}
\setres{pf.hps2}{0.304}
\setres{pf.hps3}{5.08}
\setres{pf.ir}{1.07}
\setres{pf.clip}{0.277}
\setres{pf.aes}{5.94}
\setres{pf.div}{0.214}
\setres{pf.dist}{0.280}
\setres{pf.hf}{0.92}
\setres{zbase.pick}{22.86}
\setres{zbase.hps2}{0.295}
\setres{zbase.hps3}{6.27}
\setres{zbase.ir}{0.97}
\setres{zbase.clip}{0.275}
\setres{zbase.aes}{5.42}
\setres{zbase.div}{0.155}
\setres{zpick.pick}{24.10}
\setres{zpick.hps2}{0.315}
\setres{zpick.hps3}{7.85}
\setres{zpick.ir}{1.22}
\setres{zpick.clip}{0.271}
\setres{zpick.aes}{6.06}
\setres{zpick.div}{0.116}
\setres{zpick.dist}{0.199}
\setres{zhps.pick}{23.27}
\setres{zhps.hps2}{0.357}
\setres{zhps.hps3}{9.53}
\setres{zhps.ir}{1.20}
\setres{zhps.clip}{0.275}
\setres{zhps.aes}{5.86}
\setres{zhps.div}{0.120}
\setres{zhps.dist}{0.172}
\setres{gbase1.single}{0.80}
\setres{gbase1.two}{0.30}
\setres{gbase1.count}{0.18}
\setres{gbase1.colors}{0.49}
\setres{gbase1.pos}{0.07}
\setres{gbase1.attr}{0.10}
\setres{gbase1.overall}{0.32}
\setres{gnft.single}{1.00}
\setres{gnft.two}{0.99}
\setres{gnft.count}{0.88}
\setres{gnft.colors}{0.95}
\setres{gnft.pos}{0.92}
\setres{gnft.attr}{0.86}
\setres{gnft.overall}{0.93}
\setres{gmend.single}{0.99}
\setres{gmend.two}{0.79}
\setres{gmend.count}{0.57}
\setres{gmend.colors}{0.74}
\setres{gmend.pos}{0.18}
\setres{gmend.attr}{0.47}
\setres{gmend.overall}{0.62}
\setres{gmend45.single}{1.00}
\setres{gmend45.two}{0.96}
\setres{gmend45.count}{0.69}
\setres{gmend45.colors}{0.82}
\setres{gmend45.pos}{0.32}
\setres{gmend45.attr}{0.65}
\setres{gmend45.overall}{0.74}
\setres{gfgpick.single}{1.00}
\setres{gfgpick.two}{0.94}
\setres{gfgpick.count}{0.76}
\setres{gfgpick.colors}{0.82}
\setres{gfgpick.pos}{0.27}
\setres{gfgpick.attr}{0.64}
\setres{gfgpick.overall}{0.74}
\setres{obase1.ocr}{0.13}
\setres{onft.ocr}{0.92}
\setres{omend.ocr}{0.36}
\setres{omend45.ocr}{0.53}
\setres{ofgpick.ocr}{0.68}
\setres{abbase.pick}{20.58}
\setres{abbase.div}{0.578}
\setres{abref.pick}{23.10}
\setres{abref.div}{0.297}
\setres{abkone.pick}{23.20}
\setres{abkone.div}{0.280}
\setres{abnoprice.pick}{23.21}
\setres{abnoprice.div}{0.291}
\setres{abnocap.pick}{23.27}
\setres{abnocap.div}{0.287}
\setres{abendpoint.pick}{23.34}
\setres{abendpoint.div}{0.280}
\setres{abnvone.pick}{23.16}
\setres{abnvone.div}{0.301}
\setres{abnvtwo.pick}{23.45}
\setres{abnvtwo.div}{0.260}

\setres{rwhpsv3.pick}{22.28}
\setres{rwhpsv3.hps2}{0.304}
\setres{rwhpsv3.hps3}{8.75}
\setres{rwhpsv3.ir}{0.83}
\setres{rwhpsv3.clip}{0.266}
\setres{rwhpsv3.aes}{5.95}
\setres{rwhpsv3.div}{0.310}
\setres{rwhpsv3.dist}{0.467}

